A Comprehensive Evaluation of Large Language Models on Mental Illnesses in Arabic Context

Mental health disorders pose a growing public health concern in the Arab world, emphasizing the need for accessible diagnostic and intervention tools. Large language models (LLMs) offer a promising approach, but their application in Arabic contexts faces challenges including limited labeled datasets, linguistic complexity, and translation biases. This study comprehensively evaluates 8 LLMs, including general multi-lingual models, as well as bi-lingual ones, on diverse mental health datasets (such as AraDepSu, Dreaddit, MedMCQA), investigating the impact of prompt design, language configuration (native Arabic vs. translated English, and vice versa), and few-shot prompting on diagnostic performance. We find that prompt engineering significantly influences LLM scores mainly due to reduced instruction following, with our structured prompt outperforming a less structured variant on multi-class datasets, with an average difference of 14.5\%. While language influence on performance was modest, model selection proved crucial: Phi-3.5 MoE excelled in balanced accuracy, particularly for binary classification, while Mistral NeMo showed superior performance in mean absolute error for severity prediction tasks. Few-shot prompting consistently improved performance, with particularly substantial gains observed for GPT-4o Mini on multi-class classification, boosting accuracy by an average factor of 1.58. These findings underscore the importance of prompt optimization, multilingual analysis, and few-shot learning for developing culturally sensitive and effective LLM-based mental health tools for Arabic-speaking populations.

==> ref.tex <==
% \bibliographystyle{plain}
% \bibliography{references}


\begin{thebibliography}{10}

\bibitem{who2023depression}
{World Health Organization}.
\newblock Depression, 2023.
\newblock Accessed: September 14, 2024.

\bibitem{who_anxiety}
{World Health Organization}.
\newblock Anxiety disorders, 2022.
\newblock Accessed: 2024-09-26.

\bibitem{who_mental_health_report}
{World Health Organization}.
\newblock {\em World Mental Health Report: Transforming Mental Health for All}.
\newblock World Health Organization, Geneva, 2022.
\newblock Accessed: 2024-09-26.

\bibitem{arab_barometer}
Kathrin Thomas.
\newblock Challenges of health care in the middle east and north africa.
\newblock \url{https://www.arabbarometer.org/wp-content/uploads/ABV_Health_Report_FINAL_Public-Opinion-2019.pdf}, 2019.
\newblock Arab Barometer – Wave V, Topic Report – Health Care.

\bibitem{depression_egypt_study}
Ehab~Salah Eshak and Tarek~Ahmed Abd-El~Rahman.
\newblock Depression in public servants of upper egypt: Gender-specific prevalence and determining factors.
\newblock {\em Journal of Prevention}, 43:623--638, 2022.

\bibitem{who2017depression_region}
{World Health Organization}.
\newblock Depression and other common mental disorders: Global health estimates.
\newblock \url{https://iris.who.int/bitstream/handle/10665/254610/WHO-MSD-MER-2017.2-eng.pdf?sequence=1}, 2017.
\newblock Licence: CC BY-NC-SA 3.0 IGO.

\bibitem{who2020mental_egypt}
{World Health Organization}.
\newblock Mental health atlas 2020 - member state profile: Egypt.
\newblock \url{https://cdn.who.int/media/docs/default-source/mental-health/mental-health-atlas-2020-country-profiles/egy.pdf?sfvrsn=4c708821_6&download=true}, 2020.
\newblock Licence: CC BY-NC-SA 3.0 IGO.

\bibitem{who2020mental_global}
{World Health Organization}.
\newblock Mental health atlas.
\newblock \url{https://iris.who.int/bitstream/handle/10665/345946/9789240036703-eng.pdf?sequence=1}, 2020.

\bibitem{De_Choudhury_De_2014}
Munmun De~Choudhury and Sushovan De.
\newblock Mental health discourse on reddit: Self-disclosure, social support, and anonymity.
\newblock {\em Proceedings of the International AAAI Conference on Web and Social Media}, 8(1):71--80, May 2014.

\bibitem{GUNTUKU201743}
Sharath~Chandra Guntuku, David~B Yaden, Margaret~L Kern, Lyle~H Ungar, and Johannes~C Eichstaedt.
\newblock Detecting depression and mental illness on social media: an integrative review.
\newblock {\em Current Opinion in Behavioral Sciences}, 18:43--49, 2017.
\newblock Big data in the behavioural sciences.

\bibitem{coppersmith-etal-2014-quantifying}
Glen Coppersmith, Mark Dredze, and Craig Harman.
\newblock Quantifying mental health signals in {T}witter.
\newblock In {\em Proceedings of the Workshop on Computational Linguistics and Clinical Psychology: From Linguistic Signal to Clinical Reality}, pages 51--60, Baltimore, Maryland, USA, June 2014. Association for Computational Linguistics.

\bibitem{baklola2024mental}
M~Baklola, M~Terra, A~Taha, M~Elnemr, M~Yaseen, A~Maher, AH~Buzaid, R~Alenazi, SA~Osman~Mohamed, D~Abdelhady, and AH~El-Gilany.
\newblock Mental health literacy and help-seeking behaviour among egyptian undergraduates: a cross-sectional national study.
\newblock {\em BMC Psychiatry}, 24(1):202, 2024.

\bibitem{le2021machine}
Aziliz Le~Glaz, Yannis Haralambous, Deok-Hee Kim-Dufor, Philippe Lenca, Romain Billot, Taylor~C Ryan, Jonathan Marsh, Jordan Devylder, Michel Walter, Sofian Berrouiguet, et~al.
\newblock Machine learning and natural language processing in mental health: systematic review.
\newblock {\em Journal of Medical Internet Research}, 23(5):e15708, 2021.

\bibitem{achiam2023gpt}
Josh Achiam, Steven Adler, Sandhini Agarwal, et~al.
\newblock Gpt-4 technical report.
\newblock {\em arXiv preprint arXiv:2303.08774}, 2023.

\bibitem{calvo2017natural}
Rafael~A Calvo, David~N Milne, M~Hussain, and Helen Christensen.
\newblock Natural language processing in mental health applications using large-scale text analysis.
\newblock {\em Journal of Medical Internet Research}, 19(5):e240, 2017.

\bibitem{fitzpatrick2017delivering}
Kathleen~K Fitzpatrick, Alison Darcy, and Molly Vierhile.
\newblock Delivering cognitive behavioral therapy to young adults with symptoms of depression and anxiety using a fully automated conversational agent (woebot): A randomized controlled trial.
\newblock {\em JMIR mental health}, 4(2):e19, 2017.

\bibitem{rudin2019stop}
Cynthia Rudin.
\newblock Stop explaining black box machine learning models for high stakes decisions and use interpretable models instead.
\newblock {\em Nature Machine Intelligence}, 1:206--215, 2019.

\bibitem{llm4psy}
Abdelrahman Hanafi, Mohammed Saad, Noureldin Zahran, Radwa Hanafy, and Mohammed Fouda.
\newblock A comprehensive evaluation of large language models on mental illnesses.
\newblock {\em arXiv preprint}, 2024.

\bibitem{xu2024mental}
Xuhai Xu, Bingsheng Yao, Yuanzhe Dong, Saadia Gabriel, Hong Yu, James Hendler, Marzyeh Ghassemi, Anind~K Dey, and Dakuo Wang.
\newblock Mental-llm: Leveraging large language models for mental health prediction via online text data.
\newblock {\em Proceedings of the ACM on Interactive, Mobile, Wearable and Ubiquitous Technologies}, 8(1):1--32, 2024.

\bibitem{bimedix}
Sara Pieri, Sahal~Shaji Mullappilly, Fahad~Shahbaz Khan, Rao~Muhammad Anwer, Salman Khan, Timothy Baldwin, and Hisham Cholakkal.
\newblock Bimedix: Bilingual medical mixture of experts llm.
\newblock {\em arXiv preprint arXiv:2402.13253}, 2024.

\bibitem{koubaa2024arabiangpt}
Anis Koubaa, Adel Ammar, Lahouari Ghouti, Omar Najar, and Serry Sibaee.
\newblock Arabiangpt: Native arabic gpt-based large language model, 2024.

\bibitem{DCAT}
Radwa Nassar, AbdelMoniem Helmy, and Nagy Ramadan.
\newblock Depression corpus of arabic tweets, 2022.

\bibitem{MCD}
Ashwag Maghraby and Hosnia Ali.
\newblock Modern standard arabic mood changing and depression dataset.
\newblock {\em Data in Brief}, 41:107999, 2022.

\bibitem{ARADEPSU}
Mariam Hassib, Nancy Hossam, Jolie Sameh, and Marwan Torki.
\newblock Aradepsu: Detecting depression and suicidal ideation in arabic tweets using transformers.
\newblock In {\em Proceedings of the Seventh Arabic Natural Language Processing Workshop (WANLP)}, pages 302--311. Association for Computational Linguistics, 2022.

\bibitem{CAIRODEP}
Mohammad El-Ramly, Hager Abu-Elyazid, Youseef Mo’men, Gameel Alshaer, Nardine Adib, Kareem~Alaa Eldeen, and Mariam El-Shazly.
\newblock Cairodep: Detecting depression in arabic posts using bert transformers.
\newblock In {\em 2021 Tenth International Conference on Intelligent Computing and Information Systems (ICICIS)}, pages 207--212, 2021.

\bibitem{AMI}
Arwa Diwali.
\newblock Transfer learning-based automatic sentiment annotation of a twitter-based arabic mental illness (ami) dataset, 2023.

\bibitem{MDE}
Amany~Adel Rofaida, Rofaida Ehab, Eman~Eiad Nosiba, Esraa Mahmoud, and Norhan~Abdul Menaem.
\newblock Mental health supportive application.
\newblock \url{https://github.com/esraa-mahmoudsaid/Classification-of-Mental-Disorders-in-Egyptian-dialect-of-Arabic}, 2022.
\newblock Graduation Project, Department of Medical Informatics, Faculty of Computers and Artificial Intelligence, Beni-Suef University, Egypt. Supervised by Prof. Hossam Moftah and TA Ehab Ibrahim.

\bibitem{NLLB}
NLLB Team.
\newblock No language left behind: Scaling human-centered machine translation.
\newblock {\em arXiv.2207.04672}, 2022.

\bibitem{9040556}
Norah~Saleh Alghamdi, Hanan~A. Hosni~Mahmoud, Ajith Abraham, Samar~Awadh Alanazi, and Laura García-Hernández.
\newblock Predicting depression symptoms in an arabic psychological forum.
\newblock {\em IEEE Access}, 8:57317--57334, 2020.

\bibitem{ALMOUZINI2019257}
Salma Almouzini, Maher khemakhem, and Asem Alageel.
\newblock Detecting arabic depressed users from twitter data.
\newblock {\em Procedia Computer Science}, 163:257--265, 2019.
\newblock 16th Learning and Technology Conference 2019Artificial Intelligence and Machine Learning: Embedding the Intelligence.

\bibitem{cmc.2022.022609}
Abdulqader~M. Almars.
\newblock Attention-based bi-lstm model for arabic depression classification.
\newblock {\em Computers, Materials \& Continua}, 71(2):3091--3106, 2022.

\bibitem{alabdulkreem2020}
Eatedal Alabdulkreem.
\newblock Prediction of depressed arab women using their tweets.
\newblock {\em Journal of Decision Systems}, 30(2-3):102--117, 2021.

\bibitem{turcan2019dreaddit}
Elsbeth Turcan and Kathleen McKeown.
\newblock Dreaddit: A reddit dataset for stress analysis in social media.
\newblock {\em arXiv preprint arXiv:1911.00133}, 2019.

\bibitem{haque2021deep}
Ayaan Haque, Viraaj Reddi, and Tyler Giallanza.
\newblock Deep learning for suicide and depression identification with unsupervised label correction.
\newblock In {\em Artificial Neural Networks and Machine Learning--ICANN 2021: 30th International Conference on Artificial Neural Networks, Bratislava, Slovakia, September 14--17, 2021, Proceedings, Part V 30}, pages 436--447. Springer, 2021.

\bibitem{mauriello2021sad}
Matthew~Louis Mauriello, Thierry Lincoln, Grace Hon, Dorien Simon, Dan Jurafsky, and Pablo Paredes.
\newblock Sad: A stress annotated dataset for recognizing everyday stressors in sms-like conversational systems.
\newblock In {\em Extended abstracts of the 2021 CHI conference on human factors in computing systems}, pages 1--7, 2021.

\bibitem{kabir2023deptweet}
Mohsinul Kabir, Tasnim Ahmed, Md~Bakhtiar Hasan, Md~Tahmid~Rahman Laskar, Tarun~Kumar Joarder, Hasan Mahmud, and Kamrul Hasan.
\newblock Deptweet: A typology for social media texts to detect depression severities.
\newblock {\em Computers in Human Behavior}, 139:107503, 2023.

\bibitem{sampath2022data}
Kayalvizhi Sampath and Thenmozhi Durairaj.
\newblock Data set creation and empirical analysis for detecting signs of depression from social media postings.
\newblock In {\em International Conference on Computational Intelligence in Data Science}, pages 136--151. Springer, 2022.

\bibitem{kayalvizhi2022findings}
S~Kayalvizhi, Thenmozhi Durairaj, Bharathi~Raja Chakravarthi, et~al.
\newblock Findings of the shared task on detecting signs of depression from social media.
\newblock In {\em Proceedings of the Second Workshop on Language Technology for Equality, Diversity and Inclusion}, pages 331--338, 2022.

\end{thebibliography}


